Synthesizing Control Lyapunov-Value Functions for High-Dimensional Systems Using System Decomposition and Admissible Control Sets

Control Lyapunov functions (CLFs) play a vital role in modern control applications, but finding them remains a problem. Recently, the control Lyapunov-value function (CLVF) and robust CLVF have been proposed as solutions for nonlinear time-invariant systems with bounded control and disturbance. However, the CLVF suffers from the ''curse of dimensionality,'' which hinders its application to practical high-dimensional systems. In this paper, we propose a method to decompose systems of a particular coupled nonlinear structure, in order to solve for the CLVF in each low-dimensional subsystem. We then reconstruct the full-dimensional CLVF and provide sufficient conditions for when this reconstruction is exact. Moreover, a point-wise optimal controller can be obtained using a quadratic program. We also show that when the exact reconstruction is impossible, the subsystems' CLVFs and their ``admissible control sets'' can be used to generate a Lipschitz continuous CLF. We provide several numerical examples to validate the theory and show computational efficiency.

==> backup.tex <==

\subsection{6D System}
Consider following 6D PVTOL system 
\begin{align*}
     &\dot{p_x} = v_x, \hspace{2mm} \dot{v_x} =  -F\sin{\theta}, \hspace{2mm} \dot{p_y} =  v_y,  \\ 
    &\dot{v_y} = F\cos{\theta}-g, \hspace{2mm} \dot{\theta} = \omega, \hspace{2mm} 
    % \dot{\omega} = u,  
\end{align*}
\begin{enumerate}
    \item find the ACS for all state and time for both subsystems. (ACS: $10\times 10 \times 10 \times 200 \times 2$)
    \item using repmat to make both ACS dimension match. 
    \item use ACS = intersection of the last dimension of your two sub ACSs,
\end{enumerate}
where $(p_x, p_y)$ denote the position, $(v_x, v_y)$ denote the velocity, $(\theta_x, \theta_y)$ denote the pitch and roll, and $u$ is the control input, denoting the rolling moment. $g$ is the gravitational acceleration, and $F$ is assumed to be a constant thrust moment for simplicity.

Steps for the simulation: 
\begin{enumerate}
    \item Decompose system into sub-systems, first find sub-CLVFs with $\gamma = 0$. Also find CLVF for full system. 
    \item The visFuncIm function can only plot 2D functions, the visSetIm can only project 3D, so projection is needed. 
    \item Find admissible control set for sub-systems. (You can also plot the ACS with visFuncIm/visSetIm). Back project the ACSs into original control space, take intersection of the back-proj.
    \item Back-project the sub-CLVFs into original space, use $\max(V_1,V_2)$ to reconstruct it. Compare the reconstructed CLVF with the one from original computation. 
    \item repeat above for $\gamma>0$
\end{enumerate}


\begin{align*}
     &\dot{x_1} = -x_3 \\
    &\dot{x_2} =  x_3 \\
    & \dot{x_3} = u,
\end{align*}
What we want to show: 
\begin{enumerate}
    \item Vis the set of states with empty/nonempty ACS just for the infinite-time CLVF. 
    \item starting from a state with non-empty ACS, simulate one trajectory and show it converges to the origin, and the value along it decreases exponentially
\end{enumerate}
\begin{align*}
     &\dot{x_1} = -x_2 \\
    & \dot{x_2} = u\\
\end{align*},
\begin{align*}
     &\dot{x_1} = x_2 \\
    & \dot{x_2} = u\\
\end{align*},
make sure the loss function is the infinity norm: $\ell(x) = \max_i {|x_i|}$


For both systems we need: 
\begin{enumerate}
    \item the sub CLVFs. 
    \item The reconstructed CLVF. 
    \item The original CLVF. 
    \item Keep track of the ACSS $\lim _{\tinit \rightarrow -\infty} \mathbb U(\state,\tinit)$ for both subsystems. 
\end{enumerate}

==> proofs/proof_lemma_algo.tex <==
\begin{proof}
First, we show that the ACS of the shared control for original system must be a subset of the ACS of the shared control for the subsystems. 


Next, if there exists only one admissible control signal for $\state$, then this signal can only have value on the control bound. This means the ACS 
    
\end{proof}

==> proofs/proof_prop_exactconverge.tex <==
\begin{proof}
The proof is standard and is omitted here. 
\end{proof}
